A reduced simulation applied to viscoelastic fatigue of polymers using a time multi-scale approach based on Partition of Unity method

The simulation of viscoelastic time-evolution problems described by a large number of internal variables and with a large spectrum of relaxation times requires high computational resources for their resolution. Furthermore, the internal variables evolution is described by a set of linear differential equations which involves many time scales. In this context, the use of a space-time PGD approximation is proposed here to boost their resolution, where the temporal functions are constructed following a multi-scale strategy along with the Partition of Unity method, in order to catch each dynamic efficiently. The feasibility and the robustness of the method are discussed in the case of a polymer in a non-equilibrium state under cyclic loading.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

%\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

%\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

%\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

%\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

%\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

%\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

%\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.



\bibitem{bib1} Fong, Lihwa and Advani, SG, Resin transfer molding, Handbook of Composites, Springer, 433-455, 1998.

\bibitem{bib2} Potter, Kevin D, The early history of the resin transfer moulding process for aerospace applications, Composites Part A: applied science and manufacturing, Elsevier,  619-621, 1999.


\bibitem{bib3} Zienkiewicz, Olek C and Taylor, Robert Leroy, The finite element method for solid and structural mechanics, Elsevier, 2005.


\bibitem{bib4} Smith, Gordon D and Smith, Gordon D and Smith, Gordon Dennis Smith, Numerical solution of partial differential equations: finite difference methods, Oxford university press, 1985.


\bibitem{bib5} Chinesta, Francisco and Cueto, Elias and Abisset-Chavanne, Emmanuelle and Duval, Jean Louis and Khaldi, Fouad El, Virtual, digital and hybrid twins: a new paradigm in data-based engineering and engineered data, Archives of computational methods in engineering, Springer, 105-134, 2020.





\end{thebibliography}


